The mHz quasi-regular modulations of 4U 1630--47 during its 1998 outburst

We present the results of a detailed timing and spectral analysis of the quasi-regular modulation (QRM) phenomenon in the black hole X-ray binary 4U 1630--47 during its 1998 outburst observed by Rossi X-ray Timing Explore (RXTE). We find that the $\sim$ 50-110 mHz QRM is flux dependent, and the QRM is detected with simultaneous low frequency quasi-periodic oscillations (LFQPOs). According to the behavior of the power density spectrum, we divide the observations into four groups. In the first group, namely behavior A, LFQPOs are detected, but no mHz QRM. The second group, namely behavior B, a QRM with frequency above $\sim$ 88 mHz is detected and the $\sim$ 5 Hz and $\sim$ 7 Hz LFQPOs are almost overlapping. In the third group, namely behavior C, the QRM frequency below $\sim$ 88 mHz is detected and the LFQPOs are significantly separated. In the forth group, namely behavior D, neither QRM nor LFQPOs are detected. We study the energy-dependence of the fractional rms, centroid frequency, and phase-lag of QRM and LFQPOs for behavior B and C. We then study the evolution of QRM and find that the frequency of QRM increases with hardness, while its rms decreases with hardness. We also analyze the spectra of each observation, and find that the QRM rms of behavior B has a positive correlation with $\rm F_{\rm powerlaw}$ / $\rm F_{\rm total}$. Finally, we give our understanding for this mHz QRM phenomena.

==> refer.bib/ref.tex <==


@INPROCEEDINGS{belloni_transient_2016,
       author = {{Belloni}, Tomaso M. and {Motta}, Sara E.},
        title = "{Transient Black Hole Binaries}",
     keywords = {Physics, Astrophysics - High Energy Astrophysical Phenomena},
    booktitle = {Astrophysics of Black Holes: From Fundamental Aspects to Latest Developments},
         year = 2016,
       editor = {{Bambi}, Cosimo},
       series = {Astrophysics and Space Science Library},
       volume = {440},
        month = jan,
        pages = {61},
          doi = {10.1007/978-3-662-52859-4_2},
archivePrefix = {arXiv},
       eprint = {1603.07872},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ASSL..440...61B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{homan_evolution_2005,
       author = {{Homan}, Jeroen and {Belloni}, Tomaso},
        title = "{The Evolution of Black Hole States}",
      journal = {\apss},
     keywords = {accretion, accretion disks, black hole physics, X-rays: stars, X-rays: binaries, Astrophysics},
         year = 2005,
        month = nov,
       volume = {300},
       number = {1-3},
        pages = {107-117},
          doi = {10.1007/s10509-005-1197-4},
archivePrefix = {arXiv},
       eprint = {astro-ph/0412597},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005Ap&SS.300..107H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{huppenkothen_lessttgreaterstingraylessttgreater_2019,
	title = {\${\textbackslash}less\$tt\${\textbackslash}greater\${Stingray}\${\textbackslash}less\$/tt\${\textbackslash}greater\$: {A} {Modern} \${\textbackslash}less\$tt\${\textbackslash}greater\${Python}\${\textbackslash}less\$/tt\${\textbackslash}greater\$ {Library} for {Spectral} {Timing}},
	volume = {881},
	url = {https://doi.org/10.3847/1538-4357/ab258d},
	doi = {10.3847/1538-4357/ab258d},
	abstract = {This paper describes the design and implementation of stingray, a library in Python built to perform time series analysis and related tasks on astronomical light curves. Its core functionality comprises a range of Fourier analysis techniques commonly used in spectral-timing analysis, as well as extensions for analyzing pulsar data, simulating data sets, and statistical modeling. Its modular build allows for easy extensions and incorporation of its methods into data analysis workflows and pipelines. We aim for the library to be a platform for the implementation of future spectral-timing techniques. We describe the overall vision and framework, core functionality, extensions, and connections to high-level command-line and graphical interfaces. The code is well tested, with a test coverage of currently 95\%, and is accompanied by extensive Application Program Interface (API) documentation and a set of step-by-step tutorials.},
	number = {1},
	journal = {APJ},
	author = {Huppenkothen, Daniela and Bachetti, Matteo and Stevens, Abigail L. and Migliari, Simone and Balm, Paul and Hammad, Omar and Khan, Usman Mahmood and Mishra, Himanshu and Rashid, Haroon and Sharma, Swapnil and Ribeiro, Evandro Martinez and Blanco, Ricardo Valles},
	year = {2019},
	note = {Publisher: American Astronomical Society},
	pages = {39},
}

@ARTICLE{belloni_fast_2014,
       author = {{Belloni}, Tomaso M. and {Stella}, Luigi},
        title = "{Fast Variability from Black-Hole Binaries}",
      journal = {\ssr},
     keywords = {Accretion, Accretion disks, Black hole physics, X-rays: binaries, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2014,
        month = sep,
       volume = {183},
       number = {1-4},
        pages = {43-60},
          doi = {10.1007/s11214-014-0076-0},
archivePrefix = {arXiv},
       eprint = {1407.7373},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014SSRv..183...43B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{ingram_review_2019,
       author = {{Ingram}, Adam R. and {Motta}, Sara E.},
        title = "{A review of quasi-periodic oscillations from black hole X-ray binaries: Observation and theory}",
      journal = {\nar},
     keywords = {Black holes, Neutron stars, Accretion disc, Frame-dragging, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2019,
        month = sep,
       volume = {85},
          eid = {101524},
        pages = {101524},
          doi = {10.1016/j.newar.2020.101524},
archivePrefix = {arXiv},
       eprint = {2001.08758},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019NewAR..8501524I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{casella_abc_2005,
       author = {{Casella}, P. and {Belloni}, T. and {Stella}, L.},
        title = "{The ABC of Low-Frequency Quasi-periodic Oscillations in Black Hole Candidates: Analogies with Z Sources}",
      journal = {\apj},
     keywords = {Accretion, Accretion Disks, Black Hole Physics, Stars: Oscillations, X-Rays: Binaries, Astrophysics},
         year = 2005,
        month = aug,
       volume = {629},
       number = {1},
        pages = {403-407},
          doi = {10.1086/431174},
archivePrefix = {arXiv},
       eprint = {astro-ph/0504318},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ApJ...629..403C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{ma_discovery_2021,
       author = {{Ma}, Xiang and {Tao}, Lian and {Zhang}, Shuang-Nan and {Zhang}, Liang and {Bu}, Qing-Cui and {Ge}, Ming-Yu and {Chen}, Yu-Peng and {Qu}, Jin-Lu and {Zhang}, Shu and {Lu}, Fang-Jun and {Song}, Li-Ming and {Yang}, Yi-Jung and {Yuan}, Feng and {Cai}, Ce and {Cao}, Xue-Lei and {Chang}, Zhi and {Chen}, Gang and {Chen}, Li and {Chen}, Tian-Xiang and {Chen}, Yi-Bao and {Chen}, Yong and {Cui}, Wei and {Cui}, Wei-Wei and {Deng}, Jing-Kang and {Dong}, Yong-Wei and {Du}, Yuan-Yuan and {Fu}, Min-Xue and {Gao}, Guan-Hua and {Gao}, He and {Gao}, Min and {Gu}, Yu-Dong and {Guan}, Ju and {Guo}, Cheng-Cheng and {Han}, Da-Wei and {Huang}, Yue and {Huo}, Jia and {Ji}, Long and {Jia}, Shu-Mei and {Jiang}, Lu-Hua and {Jiang}, Wei-Chun and {Jin}, Jing and {Jin}, Yong-Jie and {Kong}, Ling-Da and {Li}, Bing and {Li}, Cheng-Kui and {Li}, Gang and {Li}, Mao-Shun and {Li}, Ti-Pei and {Li}, Wei and {Li}, Xian and {Li}, Xiao-Bo and {Li}, Xu-Fang and {Li}, Yan-Guo and {Li}, Zheng-Wei and {Liang}, Xiao-Hua and {Liao}, Jin-Yuan and {Liu}, Bai-Sheng and {Liu}, Cong-Zhan and {Liu}, Guo-Qing and {Liu}, Hong-Wei and {Liu}, Xiao-Jing and {Liu}, Yi-Nong and {Lu}, Bo and {Lu}, Xue-Feng and {Luo}, Qi and {Luo}, Tao and {Meng}, Bin and {Nang}, Yi and {Nie}, Jian-Yin and {Ou}, Ge and {Sai}, Na and {Shang}, Ren-Cheng and {Song}, Xin-Ying and {Sun}, Liang and {Tan}, Ying and {Tuo}, Yuo-Li and {Wang}, Chen and {Wang}, Guo-Feng and {Wang}, Juan and {Wang}, Ling-Jun and {Wang}, Wen-Shuai and {Wang}, Yu-Sa and {Wen}, Xiang-Yang and {Wu}, Bai-Yang and {Wu}, Bo-Bing and {Wu}, Mei and {Xiao}, Guang-Cheng and {Xiao}, Shuo and {Xie}, Fu-Guo and {Xiong}, Shao-Lin and {Xu}, He and {Xu}, Yu-Peng and {Yang}, Jia-Wei and {Yang}, Sheng and {Yang}, Yan-Ji and {Yi}, Qi-Bin and {Yin}, Qian-Qing and {You}, Yuan and {Zhang}, Ai-Mei and {Zhang}, Cheng-Mo and {Zhang}, Fan and {Zhang}, Hong-Mei and {Zhang}, Juan and {Zhang}, Tong and {Zhang}, Wan-Chang and {Zhang}, Wei and {Zhang}, Wen-Zhao and {Zhang}, Yi and {Zhang}, Yi-Fei and {Zhang}, Yong-Jie and {Zhang}, Yue and {Zhang}, Zhao and {Zhang}, Zhi and {Zhang}, Zi-Liang and {Zhao}, Hai-Sheng and {Zhao}, Xiao-Fan and {Zheng}, Shi-Jie and {Zhou}, Deng-Ke and {Zhou}, Jian-Feng and {Zhu}, Yu-Xuan and {Zhu}, Yue and {Zhuang}, Ren-Lin},
        title = "{Discovery of oscillations above 200 keV in a black hole X-ray binary with Insight-HXMT}",
      journal = {Nature Astronomy},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena},
         year = 2021,
        month = jan,
       volume = {5},
        pages = {94-102},
          doi = {10.1038/s41550-020-1192-2},
archivePrefix = {arXiv},
       eprint = {2009.10607},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021NatAs...5...94M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{ingram_low-frequency_2009,
       author = {{Ingram}, Adam and {Done}, Chris and {Fragile}, P. Chris},
        title = "{Low-frequency quasi-periodic oscillations spectra and Lense-Thirring precession}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, black hole physics, X-rays: binaries, Astrophysics - Solar and Stellar Astrophysics},
         year = 2009,
        month = jul,
       volume = {397},
       number = {1},
        pages = {L101-L105},
          doi = {10.1111/j.1745-3933.2009.00693.x},
archivePrefix = {arXiv},
       eprint = {0901.1238},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009MNRAS.397L.101I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{trudolyubov_rxte_2001,
       author = {{Trudolyubov}, Sergey P. and {Borozdin}, Konstantin N. and {Priedhorsky}, William C.},
        title = "{RXTE observations of 4U 1630-47 during the peak of its 1998 outburst}",
      journal = {\mnras},
     keywords = {BLACK HOLE PHYSICS, BINARIES: GENERAL, STARS: INDIVIDUAL: 4U 1630-47, NOVAE, CATACLYSMIC VARIABLES, X-RAYS: GENERAL, Astrophysics},
         year = 2001,
        month = apr,
       volume = {322},
       number = {2},
        pages = {309-320},
          doi = {10.1046/j.1365-8711.2001.04073.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/9911345},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001MNRAS.322..309T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{altamirano_low-frequency_2012,
       author = {{Altamirano}, D. and {Strohmayer}, T.},
        title = "{Low-frequency (11 mHz) Oscillations in H1743-322: A New Class of Black Hole Quasi-periodic Oscillations?}",
      journal = {\apjl},
     keywords = {binaries: close, black hole physics, stars: individual: H1743-322, X-rays: binaries, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2012,
        month = aug,
       volume = {754},
       number = {2},
          eid = {L23},
        pages = {L23},
          doi = {10.1088/2041-8205/754/2/L23},
archivePrefix = {arXiv},
       eprint = {1206.0476},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...754L..23A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{zhang_z_variability_2014,
       author = {{Zhang}, Z. and {Qu}, J.~L. and {Gao}, H.~Q. and {Zhang}, S. and {Bu}, Q.~C. and {Ge}, M.~Y. and {Chen}, L. and {Li}, Z.~B.},
        title = "{The variability classes in IGR J17091-3624 during the 2011 outburst}",
      journal = {\aap},
     keywords = {stars: individual: IGR J17091, 3624, X-rays: binaries, accretion, accretion disks, black hole physics},
         year = 2014,
        month = sep,
       volume = {569},
          eid = {A33},
        pages = {A33},
          doi = {10.1051/0004-6361/201323294},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014A&A...569A..33Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{morgan_lessigreaterrxtelessigreaterobservations_1997,
       author = {{Morgan}, E.~H. and {Remillard}, R.~A. and {Greiner}, J.},
        title = "{RXTE Observations of QPOs in the Black Hole Candidate GRS 1915+105}",
      journal = {\apj},
     keywords = {Black Hole Physics, Stars: Individual: Alphanumeric: GRS 1915+105, Stars: Oscillations, X-Rays: Stars},
         year = 1997,
        month = jun,
       volume = {482},
       number = {2},
        pages = {993-1010},
          doi = {10.1086/304191},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997ApJ...482..993M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{remillard_lessigreaterrxtelessigreaterobservations_1999,
       author = {{Remillard}, Ronald A. and {Morgan}, Edward H. and {McClintock}, Jeffrey E. and {Bailyn}, Charles D. and {Orosz}, Jerome A.},
        title = "{RXTE Observations of 0.1-300 HZ Quasi-periodic Oscillationsin the Microquasar GRO J1655-40}",
      journal = {\apj},
     keywords = {BLACK HOLE PHYSICS, STARS: INDIVIDUAL: ALPHANUMERIC: GRO J1655-40, STARS: OSCILLATIONS, X-RAYS: STARS, Black Hole Physics, Stars: Individual: Alphanumeric: GRO J1655-40, Stars: Oscillations, X-Rays: Stars},
         year = 1999,
        month = sep,
       volume = {522},
       number = {1},
        pages = {397-412},
          doi = {10.1086/307606},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999ApJ...522..397R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{priedhorsky_recurrent_1986,
       author = {{Priedhorsky}, W.},
        title = "{Recurrent Population II X-ray transients {\textemdash} similarities to SU UMa cataclysmic variables}",
      journal = {\apss},
     keywords = {Cataclysmic Variables, X Ray Binaries, Fourier Transformation, Light Curve, Mass Transfer, Temporal Distribution, Astrophysics},
         year = 1986,
        month = oct,
       volume = {126},
       number = {1},
        pages = {89-98},
          doi = {10.1007/BF00644177},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1986Ap&SS.126...89P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{choudhury_qpo_2015,
       author = {{Choudhury}, Manojendu and {Bhatt}, Nilay and {Bhattacharyya}, Subir},
        title = "{The QPO states of 4U 1630-47}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, black hole physics, stars: individual: 4U 1630-47, X-rays: binaries, X-rays: individual: 4U 1630-47, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2015,
        month = mar,
       volume = {447},
       number = {4},
        pages = {3960-3972},
          doi = {10.1093/mnras/stu2742},
archivePrefix = {arXiv},
       eprint = {1502.01432},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.447.3960C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{tetarenko_watchdog_2016,
       author = {{Tetarenko}, B.~E. and {Sivakoff}, G.~R. and {Heinke}, C.~O. and {Gladstone}, J.~C.},
        title = "{WATCHDOG: A Comprehensive All-sky Database of Galactic Black Hole X-ray Binaries}",
      journal = {\apjs},
     keywords = {accretion, accretion disks, black hole physics, catalogs, stars: black holes, X-rays: binaries, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2016,
        month = feb,
       volume = {222},
       number = {2},
          eid = {15},
        pages = {15},
          doi = {10.3847/0067-0049/222/2/15},
archivePrefix = {arXiv},
       eprint = {1512.00778},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJS..222...15T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1991ApJ...383..784M,
       author = {{Miyamoto}, Sigenori and {Kimura}, Kazuhiro and {Kitamoto}, Shunji and {Dotani}, Tadayasu and {Ebisawa}, Ken},
        title = "{X-Ray Variability of GX 339-4 in Its Very High State}",
      journal = {\apj},
     keywords = {Stellar Spectra, X Ray Binaries, X Ray Spectra, Black Body Radiation, Energy Spectra, Spectrum Analysis, X Ray Astronomy, Astrophysics, STARS: INDIVIDUAL ALPHANUMERIC: GX 339-4, X-RAYS: BINARIES, X-RAYS: SPECTRA},
         year = 1991,
        month = dec,
       volume = {383},
        pages = {784},
          doi = {10.1086/170837},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1991ApJ...383..784M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{1997ApJ...479..926M,
       author = {{M{\'e}ndez}, Mariano and {van der Klis}, Michiel},
        title = "{The EXOSAT Data on GX 339-4: Further Evidence for an ``Intermediate'' State}",
      journal = {\apj},
     keywords = {Stars: Binaries: Close, Black Hole Physics, Stars: Individual: Alphanumeric: GX 330-4, X-Rays: Stars, Astrophysics},
         year = 1997,
        month = apr,
       volume = {479},
       number = {2},
        pages = {926-932},
          doi = {10.1086/303914},
archivePrefix = {arXiv},
       eprint = {astro-ph/9611015},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997ApJ...479..926M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{parmar_periodic_1995,
       author = {{Parmar}, A.~N. and {Angelini}, L. and {White}, N.~E.},
        title = "{Periodic Outbursts from the Ultrasoft X-Ray Transient 4U 1630-47}",
      journal = {\apjl},
     keywords = {ACCRETION, ACCRETION DISKS, STARS: BINARIES: CLOSE, STARS: INDIVIDUAL ALPHANUMERIC: 4U 1630-47, X-RAYS: STARS},
         year = 1995,
        month = oct,
       volume = {452},
        pages = {L129},
          doi = {10.1086/309730},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995ApJ...452L.129P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{seifina_black_2014,
       author = {{Seifina}, Elena and {Titarchuk}, Lev and {Shaposhnikov}, Nikolai},
        title = "{Black Hole Mass Determination in the X-Ray Binary 4U 1630-47: Scaling of Spectral and Variability Characteristics}",
      journal = {\apj},
     keywords = {accretion, accretion disks, black hole physics, radiation mechanisms: non-thermal, stars: individual: 4U 1630-47, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2014,
        month = jul,
       volume = {789},
       number = {1},
          eid = {57},
        pages = {57},
          doi = {10.1088/0004-637X/789/1/57},
archivePrefix = {arXiv},
       eprint = {1405.4711},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...789...57S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tomsick_x-ray_1998,
       author = {{Tomsick}, J.~A. and {Lapshov}, I. and {Kaaret}, P.},
        title = "{An X-Ray Dip in the X-Ray Transient 4U 1630-47}",
      journal = {\apj},
     keywords = {ACCRETION, ACCRETION DISKS, BLACK HOLE PHYSICS, STARS: INDIVIDUAL ALPHANUMERIC: 4U 1630-47, X-RAYS: STARS, Accretion, Accretion Disks, Black Hole Physics, Stars: Individual: Alphanumeric: 4U 1630-47, X-Rays: Stars, Astrophysics},
         year = 1998,
        month = feb,
       volume = {494},
       number = {2},
        pages = {747-752},
          doi = {10.1086/305240},
archivePrefix = {arXiv},
       eprint = {astro-ph/9709214},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998ApJ...494..747T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{king_disk_2014,
       author = {{King}, Ashley L. and {Walton}, Dominic J. and {Miller}, Jon M. and {Barret}, Didier and {Boggs}, Steven E. and {Christensen}, Finn E. and {Craig}, William W. and {Fabian}, Andy C. and {F{\"u}rst}, Felix and {Hailey}, Charles J. and {Harrison}, Fiona A. and {Krivonos}, Roman and {Mori}, Kaya and {Natalucci}, Lorenzo and {Stern}, Daniel and {Tomsick}, John A. and {Zhang}, William W.},
        title = "{The Disk Wind in the Rapidly Spinning Stellar-mass Black Hole 4U 1630-472 Observed with NuSTAR}",
      journal = {\apjl},
     keywords = {accretion, accretion disks, black hole physics, stars: winds, outflows, X-rays: binaries, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2014,
        month = mar,
       volume = {784},
       number = {1},
          eid = {L2},
        pages = {L2},
          doi = {10.1088/2041-8205/784/1/L2},
archivePrefix = {arXiv},
       eprint = {1401.3646},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...784L...2K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{baby_astrosat_2020,
       author = {{Baby}, Blessy E. and {Agrawal}, V.~K. and {Ramadevi}, M.~C. and {Katoch}, Tilak and {Antia}, H.~M. and {Mandal}, Samir and {Nandi}, Anuj},
        title = "{AstroSat and MAXI view of the black hole binary 4U 1630-472 during 2016 and 2018 outbursts}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, black hole physics, stars: individual: 4U 1630-47, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = sep,
       volume = {497},
       number = {1},
        pages = {1197-1211},
          doi = {10.1093/mnras/staa1965},
archivePrefix = {arXiv},
       eprint = {2007.00928},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.497.1197B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{belloni_unified_2002,
       author = {{Belloni}, Tomaso and {Psaltis}, Dimitrios and {van der Klis}, Michiel},
        title = "{A Unified Description of the Timing Features of Accreting X-Ray Binaries}",
      journal = {\apj},
     keywords = {Accretion, Accretion Disks, Black Hole Physics, Stars: Neutron, Stars: Oscillations, X-Rays: Stars, Astrophysics},
         year = 2002,
        month = jun,
       volume = {572},
       number = {1},
        pages = {392-406},
          doi = {10.1086/340290},
archivePrefix = {arXiv},
       eprint = {astro-ph/0202213},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002ApJ...572..392B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{belloni_atlas_1990,
       author = {{Belloni}, T. and {Hasinger}, G.},
        title = "{An atlas of aperiodic variability in HMXB.}",
      journal = {\aap},
     keywords = {Pulsars, Stellar Spectra, Variable Stars, X Ray Binaries, Black Holes (Astronomy), Color-Color Diagram, Power Spectra, Astrophysics},
         year = 1990,
        month = apr,
       volume = {230},
        pages = {103-119},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1990A&A...230..103B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{miyamoto_x-ray_1991,
	title = {X-{Ray} {Variability} of {GX} 339-4 in {Its} {Very} {High} {State}},
	volume = {383},
	doi = {10.1086/170837},
	journal = {{\apj},
	author = {Miyamoto, Sigenori and Kimura, Kazuhiro and Kitamoto, Shunji and Dotani, Tadayasu and Ebisawa, Ken},
	month = dec,
	year = {1991},
	keywords = {Astrophysics, Stellar Spectra, X Ray Binaries, Black Body Radiation, Energy Spectra, Spectrum Analysis, STARS: INDIVIDUAL ALPHANUMERIC: GX 339-4, X Ray Astronomy, X Ray Spectra, X-RAYS: BINARIES, X-RAYS: SPECTRA},
	pages = {784},
}}

@ARTICLE{2015ApJ...799....2B,
       author = {{Bu}, Qing-cui and {Chen}, Li and {Li}, Zhao-sheng and {Qu}, Jin-lu and {Belloni}, T.~M. and {Zhang}, Liang},
        title = "{Correlations in Horizontal Branch Oscillations and Break Components in XTE J1701-462 and GX 17+2}",
      journal = {\apj},
     keywords = {accretion, accretion disks, black hole physics, stars: general, stars: neutron, X-rays: binaries, X-rays: stars, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2015,
        month = jan,
       volume = {799},
       number = {1},
          eid = {2},
        pages = {2},
          doi = {10.1088/0004-637X/799/1/2},
archivePrefix = {arXiv},
       eprint = {1411.1137},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...799....2B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{reig_phase_2000,
       author = {{Reig}, P. and {Belloni}, T. and {van der Klis}, M. and {M{\'e}ndez}, M. and {Kylafis}, N.~D. and {Ford}, E.~C.},
        title = "{Phase Lag Variability Associated with the 0.5-10 HZ Quasi-Periodic Oscillations in GRS 1915+105}",
      journal = {\apj},
     keywords = {Accretion, Accretion Disks, stars: individual (GRS 1915+105), Stars: Neutron, X-Rays: Stars},
         year = 2000,
        month = oct,
       volume = {541},
       number = {2},
        pages = {883-888},
          doi = {10.1086/309469},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...541..883R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{kong_joint_2020,
       author = {{Kong}, L.~D. and {Zhang}, S. and {Chen}, Y.~P. and {Ji}, L. and {Zhang}, S.~N. and {Yang}, Y.~R. and {Tao}, L. and {Ma}, X. and {Qu}, J.~L. and {Lu}, F.~J. and {Bu}, Q.~C. and {Chen}, L. and {Song}, L.~M. and {Li}, T.~P. and {Xu}, Y.~P. and {Cao}, X.~L. and {Chen}, Y. and {Liu}, C.~Z. and {Cai}, C. and {Chang}, Z. and {Chen}, G. and {Chen}, T.~X. and {Chen}, Y.~B. and {Cui}, W. and {Cui}, W.~W. and {Deng}, J.~K. and {Dong}, Y.~W. and {Du}, Y.~Y. and {Fu}, M.~X. and {Gao}, G.~H. and {Gao}, H. and {Gao}, M. and {Ge}, M.~Y. and {Gu}, Y.~D. and {Guan}, J. and {Guo}, C.~C. and {Han}, D.~W. and {Huang}, Y. and {Huo}, J. and {Jia}, S.~M. and {Jiang}, L.~H. and {Jiang}, W.~C. and {Jin}, J. and {Li}, B. and {Li}, C.~K. and {Li}, G. and {Li}, M.~S. and {Li}, W. and {Li}, X. and {Li}, X.~B. and {Li}, X.~F. and {Li}, Y.~G. and {Li}, Z.~W. and {Liang}, X.~H. and {Liao}, J.~Y. and {Liu}, G.~Q. and {Liu}, H.~X. and {Liu}, H.~W. and {Liu}, S.~Z. and {Liu}, X.~J. and {Liu}, Y.~N. and {Lu}, B. and {Lu}, X.~F. and {Luo}, Q. and {Luo}, T. and {Meng}, B. and {Nang}, Y. and {Nie}, J.~Y. and {Ou}, G. and {Ren}, X.~Q. and {Sai}, N. and {Song}, X.~Y. and {Sun}, L. and {Tan}, Y. and {Tuo}, Y.~L. and {Wang}, C. and {Wang}, G.~F. and {Wang}, J. and {Wang}, P.~J. and {Wang}, W.~S. and {Wang}, Y.~S. and {Wen}, X.~Y. and {Wu}, B.~Y. and {Wu}, B.~B. and {Wu}, M. and {Xiao}, G.~C. and {Xiao}, S. and {Xiong}, S.~L. and {Xu}, H. and {Yang}, J.~W. and {Yang}, S. and {Yang}, Y.~J. and {Yi}, Q.~B. and {You}, Y. and {Zhang}, A.~M. and {Zhang}, C.~M. and {Zhang}, F. and {Zhang}, H.~M. and {Zhang}, J. and {Zhang}, P. and {Zhang}, T. and {Zhang}, W. and {Zhang}, W.~C. and {Zhang}, W.~Z. and {Zhang}, Y. and {Zhang}, Y.~F. and {Zhang}, Y.~J. and {Zhang}, Y.~H. and {Zhang}, Y. and {Zhang}, Z. and {Zhang}, Z.~L. and {Zhao}, H.~S. and {Zhao}, X.~F. and {Zheng}, S.~J. and {Zheng}, Y.~G. and {Zhou}, D.~K. and {Zhou}, J.~F. and {Zhu}, Y.~X. and {Zhu}, Y. and {Insight-HXMT Collaboration}},
        title = "{Joint analysis of energy and RMS spectra from MAXI J1535-571 with Insight-HXMT}",
      journal = {JHEA},
     keywords = {Starts: individual (MAXI J1535-571), X-rays: binaries, Black hole physics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = mar,
       volume = {25},
        pages = {29-38},
          doi = {10.1016/j.jheap.2020.01.003},
archivePrefix = {arXiv},
       eprint = {2001.06637},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020JHEAp..25...29K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{fender_jets_2009,
       author = {{Fender}, R.~P. and {Homan}, J. and {Belloni}, T.~M.},
        title = "{Jets from black hole X-ray binaries: testing, refining and extending empirical models for the coupling to X-rays}",
      journal = {\mnras},
     keywords = {ISM: jets and outflows, radio continuum: stars, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2009,
        month = jul,
       volume = {396},
       number = {3},
        pages = {1370-1382},
          doi = {10.1111/j.1365-2966.2009.14841.x},
archivePrefix = {arXiv},
       eprint = {0903.5166},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009MNRAS.396.1370F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{mendez_exosat_1997,
	title = {The {EXOSAT} {Data} on {GX} 339-4: {Further} {Evidence} for an “{Intermediate}” {State}},
	volume = {479},
	doi = {10.1086/303914},
	number = {2},
	journal = {{\apj},
	author = {Méndez, Mariano and van der Klis, Michiel},
	month = apr,
	year = {1997},
	note = {\_eprint: astro-ph/9611015},
	keywords = {Astrophysics, Black Hole Physics, Stars: Binaries: Close, Stars: Individual: Alphanumeric: GX 330-4, X-Rays: Stars},
	pages = {926--932},
}
}

@article{van_der_klis_similarities_1994, 
	title = {Similarities in {Neutron} {Star} and {Black} {Hole} {Accretion}},
	volume = {92},
	doi = {10.1086/192006},
	journal = {{\apjs},
	author = {van der Klis, M.},
	month = jun,
	year = {1994},
	keywords = {Black Holes (Astronomy), Color-Color Diagram, Power Spectra, X Ray Binaries, X Ray Astronomy, X Ray Spectra, ACCRETION, ACCRETION DISKS, Astronomy, BLACK HOLE PHYSICS, Light Curve, Neutron Stars, STARS: NEUTRON, Stellar Mass Accretion, Stellar Oscillations},
	pages = {511},}
}

@INPROCEEDINGS{van_der_klis_fourier_1989,
       author = {{van der Klis}, M.},
        title = "{Fourier techniques in X-ray timing}",
     keywords = {X-Ray Pulsars: Periods, X-Ray Pulsars: Power Spectra},
    booktitle = {Timing Neutron Stars},
         year = 1989,
       editor = {{{\"O}gelman}, H. and {van den Heuvel}, E.~P.~J.},
       series = {NATO Advanced Study Institute (ASI) Series C},
       volume = {262},
        month = jan,
        pages = {27},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1989ASIC..262...27V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{belloni_unified_2002-1,
	title = {A {Unified} {Description} of the {Timing} {Features} of {Accreting} {X}-{Ray} {Binaries}},
	volume = {572},
	url = {https://doi.org/10.1086/340290},
	doi = {10.1086/340290},
	abstract = {We study an empirical model for a unified description of the power spectra of accreting neutron stars and black holes. This description is based on a superposition of multiple Lorentzians and offers the advantage that all quasi-periodic oscillation and noise components are dealt with in the same way, without the need of deciding in advance the nature of each component. This approach also allows us to compare frequencies of features with high and low coherences in a consistent manner and greatly facilitates comparison of power spectra across a wide range of source types and states. We apply the model to six sources: the low-luminosity X-ray bursters 1E 1724-3045, SLX 1735-269, and GS 1826-24; the high-latitude transient XTE J1118+480; the bright system Cir X-1; and the Z source GX 17+2. We find that it provides a good description of the observed spectra without the need for a scale-free (1/f) component. We update previously reported correlations between characteristic frequencies of timing features in the light of this new approach and discuss similarities between different types of systems that may point toward similar underlying physics.},
	number = {1},
	journal = {\apj},
	author = {Belloni, Tomaso and Psaltis, Dimitrios and Klis, Michiel van der},
	month = jun,
	year = {2002},
	note = {Publisher: American Astronomical Society},
	pages = {392--406},
}

@ARTICLE{nowak_are_2000,
       author = {{Nowak}, M.~A.},
        title = "{Are there three peaks in the power spectra of GX 339-4 and Cyg X-1?}",
      journal = {\mnras},
     keywords = {ACCRETION, ACCRETION DISCS, BLACK HOLE PHYSICS, BINARIES: GENERAL, STARS: INDIVIDUAL: CYG X-1, STARS: INDIVIDUAL: GX339-4, X-RAYS: STARS, Astrophysics},
         year = 2000,
        month = oct,
       volume = {318},
       number = {2},
        pages = {361-367},
          doi = {10.1046/j.1365-8711.2000.03668.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0005232},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000MNRAS.318..361N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{ingram_review_2019-1,
	title = {A review of quasi-periodic oscillations from black hole {X}-ray binaries: {Observation} and theory},
	volume = {85},
	doi = {10.1016/j.newar.2020.101524},
	journal = {{\textbackslash}nar},
	author = {Ingram, Adam R. and Motta, Sara E.},
	month = sep,
	year = {2019},
	note = {\_eprint: 2001.08758},
	keywords = {Accretion disc, Black holes, Frame-dragging, Neutron stars, Astrophysics - High Energy Astrophysical Phenomena},
	pages = {101524},
}

@ARTICLE{van_der_klis_qpo_2005,
       author = {{van der Klis}, M.},
        title = "{The QPO phenomenon}",
      journal = {Astronomische Nachrichten},
     keywords = {stars: neutron, black hole physics, quasi-periodic oscillations},
         year = 2005,
        month = nov,
       volume = {326},
       number = {9},
        pages = {798-803},
          doi = {10.1002/asna.200510416},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005AN....326..798V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{ingram_physical_2010,
	title = {A physical interpretation of the variability power spectral components in accreting neutron stars},
	volume = {405},
	issn = {0035-8711},
	url = {https://doi.org/10.1111/j.1365-2966.2010.16614.x},
	doi = {10.1111/j.1365-2966.2010.16614.x},
	abstract = {We propose a physical framework for interpreting the characteristic frequencies seen in the broad-band power spectra from black hole and neutron star binaries. We use the truncated disc/hot inner flow geometry, and assume that the hot flow is generically turbulent. Each radius in the hot flow produces fluctuations, and we further assume that these are damped on the viscous frequency. Integrating over radii gives broad-band continuum noise power between low- and high-frequency breaks which are set by the viscous time-scale at the outer and inner edge of the hot flow, respectively. Lense–Thirring (vertical) precession of the entire hot flow superimposes the low-frequency quasi-periodic oscillation (QPO) on this continuum power.We test this model on the power spectra seen in the neutron star systems (atolls) as these have the key advantage that the (upper) kHz QPO most likely independently tracks the truncation radius. These show that this model can give a consistent solution, with the truncation radius decreasing from 20 to 8 Rg while the inner radius of the flow remains approximately constant at ∼4.5 Rg i.e. 9.2 km. We use this very constrained geometry to predict the low-frequency QPO from Lense–Thirring precession of the entire hot flow from ro to ri. The simplest assumption of a constant surface density in the hot flow matches the observed QPO frequency to within 25 per cent. This match can be made even better by considering that the surface density should become increasingly centrally concentrated as the flow collapses into an optically thick boundary layer during the spectral transition. The success of the model opens up the way to use the broad-band power spectra as a diagnostic of accretion flows in strong gravity.},
	number = {4},
	journal = {\mnras},
	author = {Ingram, Adam and Done, Chris},
	month = jul,
	year = {2010},
	note = {\_eprint: https://academic.oup.com/mnras/article-pdf/405/4/2447/18437976/mnras0405-2447.pdf},
	pages = {2447--2452},
}


@ARTICLE{ingram_physical_2011,
       author = {{Ingram}, Adam and {Done}, Chris},
        title = "{A physical model for the continuum variability and quasi-periodic oscillation in accreting black holes}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, X-rays: binaries, X-rays: individual: XTE J1550-584, Astrophysics - Solar and Stellar Astrophysics},
         year = 2011,
        month = aug,
       volume = {415},
       number = {3},
        pages = {2323-2335},
          doi = {10.1111/j.1365-2966.2011.18860.x},
archivePrefix = {arXiv},
       eprint = {1101.2336},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011MNRAS.415.2323I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{zhang_evolution_2017,
	title = {The {Evolution} of the {Phase} {Lags} {Associated} with the {Type}-{C} {Quasi}-periodic {Oscillation} in {GX} 339-4 during the 2006/2007 {Outburst}},
	volume = {845},
	doi = {10.3847/1538-4357/aa8138},
	number = {2},
	journal = {{\apj},
	author = {Zhang, Liang and Wang, Yanan and Méndez, Mariano and Chen, Li and Qu, Jinlu and Altamirano, Diego and Belloni, Tomaso},
	month = aug,
	year = {2017},
	note = {\_eprint: 1707.06228},
	keywords = {X-rays: binaries, Astrophysics - High Energy Astrophysical Phenomena, black hole physics, accretion, accretion disks},
	pages = {143},
}
}

@article{lyu_xmm-newton_2020,
	title = {{XMM}-{Newton} and {NICER} {Measurement} of the {Rms} {Spectrum} of the {Millihertz} {Quasiperiodic} {Oscillations} in the {Neutron}-star {Low}-mass {X}-{Ray} {Binary} {4U} 1636-53},
	volume = {895},
	doi = {10.3847/1538-4357/ab8cbe},
	number = {2},
	journal = {{\apj},
	author = {Lyu, Ming and Zhang, Guobao and Méndez, Mariano and Altamirano, D. and Mancuso, G. C. and Xiang, Fu-Yuan and Xiao, Huaping},
	month = jun,
	year = {2020},
	note = {\_eprint: 2006.09563},
	keywords = {Neutron stars, Astrophysics - High Energy Astrophysical Phenomena, 100, 1108, 939, Astrophysical explosive burning, Low-mass x-ray binary stars},
	pages = {120},
}
}
@ARTICLE{2020ApJ...895..120L,
       author = {{Lyu}, Ming and {Zhang}, Guobao and {M{\'e}ndez}, Mariano and {Altamirano}, D. and {Mancuso}, G.~C. and {Xiang}, Fu-Yuan and {Xiao}, Huaping},
        title = "{XMM-Newton and NICER Measurement of the Rms Spectrum of the Millihertz Quasiperiodic Oscillations in the Neutron-star Low-mass X-Ray Binary 4U 1636-53}",
      journal = {\apj},
     keywords = {Low-mass x-ray binary stars, Neutron stars, Astrophysical explosive burning, 939, 1108, 100, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = jun,
       volume = {895},
       number = {2},
          eid = {120},
        pages = {120},
          doi = {10.3847/1538-4357/ab8cbe},
archivePrefix = {arXiv},
       eprint = {2006.09563},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...895..120L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{lyu_xmm-newton_2020-1,
	title = {{XMM}-{Newton} and {NICER} {Measurement} of the {Rms} {Spectrum} of the {Millihertz} {Quasiperiodic} {Oscillations} in the {Neutron}-star {Low}-mass {X}-{Ray} {Binary} {4U} 1636-53},
	volume = {895},
	doi = {10.3847/1538-4357/ab8cbe},
	number = {2},
	journal = {{\apj},
	author = {Lyu, Ming and Zhang, Guobao and Méndez, Mariano and Altamirano, D. and Mancuso, G. C. and Xiang, Fu-Yuan and Xiao, Huaping},
	month = jun,
	year = {2020},
	note = {\_eprint: 2006.09563},
	keywords = {Neutron stars, Astrophysics - High Energy Astrophysical Phenomena, 100, 1108, 939, Astrophysical explosive burning, Low-mass x-ray binary stars},
	pages = {120},
}
}

@ARTICLE{2022MNRAS.512.2082L,
       author = {{Liu}, Qichun and {Liu}, Honghui and {Bambi}, Cosimo and {Ji}, Long},
        title = "{The spins of the Galactic black holes in MAXI J1535-571 and 4U 1630-472 from Insight-HXMT}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, black hole physics, Astrophysics - High Energy Astrophysical Phenomena, General Relativity and Quantum Cosmology},
         year = 2022,
        month = may,
       volume = {512},
       number = {2},
        pages = {2082-2092},
          doi = {10.1093/mnras/stac616},
archivePrefix = {arXiv},
       eprint = {2111.00719},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.512.2082L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{capitanio_missing_2015,
       author = {{Capitanio}, F. and {Campana}, R. and {De Cesare}, G. and {Ferrigno}, C.},
        title = "{Missing hard states and regular outbursts: the puzzling case of the black hole candidate 4U 1630-472}",
      journal = {\mnras},
     keywords = {black hole physics, methods: data analysis, binaries: close, stars: black holes, X-rays: binaries, X-rays: individual: 4U1630-472, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2015,
        month = jul,
       volume = {450},
       number = {4},
        pages = {3840-3854},
          doi = {10.1093/mnras/stv687},
archivePrefix = {arXiv},
       eprint = {1505.04034},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.450.3840C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2022MNRAS.514.5238M,
       author = {{Ma}, R.~C. and {Soria}, R. and {Tao}, L. and {Zhang}, W. and {Qu}, J.~L. and {Zhang}, S.~N. and {Zhang}, L. and {Qiao}, E.~L. and {Zhao}, S.~J. and {Ge}, M.~Y. and {Li}, X.~B. and {Huang}, Y. and {Song}, L.~M. and {Zhang}, S. and {Bu}, Q.~C. and {Wang}, Y.~N. and {Ma}, X. and {Jia}, S.~M.},
        title = "{The peculiar spectral evolution of the new X-ray transient MAXI J0637-430}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, X-rays: binaries, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2022,
        month = aug,
       volume = {514},
       number = {4},
        pages = {5238-5265},
          doi = {10.1093/mnras/stac1585},
archivePrefix = {arXiv},
       eprint = {2206.03409},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.514.5238M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{dieters_timing_2000,
       author = {{Dieters}, S.~W. and {Belloni}, T. and {Kuulkers}, E. and {Woods}, P. and {Cui}, W. and {Zhang}, S.~N. and {Chen}, W. and {van der Klis}, M. and {van Paradijs}, J. and {Swank}, J. and {Lewin}, W.~H.~G. and {Kouveliotou}, C.},
        title = "{The Timing Evolution of 4U 1630-47 during Its 1998 Outburst}",
      journal = {\apj},
     keywords = {Accretion, Accretion Disks, Stars: Binaries: Close, stars: individual (4U 1630-47), X-Rays: Stars, Astrophysics},
         year = 2000,
        month = jul,
       volume = {538},
       number = {1},
        pages = {307-314},
          doi = {10.1086/309108},
archivePrefix = {arXiv},
       eprint = {astro-ph/9912028},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...538..307D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{tomsick_x-ray_2000,
       author = {{Tomsick}, John A. and {Kaaret}, Philip},
        title = "{X-Ray Spectral and Timing Evolution during the Decay of the 1998 Outburst from the Recurrent X-Ray Transient 4U 1630-47}",
      journal = {\apj},
     keywords = {Accretion, Accretion Disks, Black Hole Physics, stars: individual (4U 1630-47), X-Rays: Bursts, X-Rays: Stars, Astrophysics},
         year = 2000,
        month = jul,
       volume = {537},
       number = {1},
        pages = {448-460},
          doi = {10.1086/308999},
archivePrefix = {arXiv},
       eprint = {astro-ph/0002084},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...537..448T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{pasham_nature_2013,
	title = {On the {Nature} of the {mHz} {X}-{Ray} {Quasi}-periodic {Oscillations} from {Ultraluminous} {X}-{Ray} {Source} {M82} {X}-1: {Search} for {Timing}-{Spectral} {Correlations}},
	volume = {771},
	doi = {10.1088/0004-637X/771/2/101},
	number = {2},
	journal = {{\apj},
	author = {Pasham, Dheeraj R. and Strohmayer, Tod E.},
	month = jul,
	year = {2013},
	note = {\_eprint: 1308.1677},
	keywords = {X-rays: binaries, Astrophysics - High Energy Astrophysical Phenomena, accretion, accretion disks, methods: data analysis},
	pages = {101},
}
}

@ARTICLE{qu_energy_2010,
       author = {{Qu}, J.~L. and {Lu}, F.~J. and {Lu}, Y. and {Song}, L.~M. and {Zhang}, S. and {Ding}, G.~Q. and {Wang}, J.~M.},
        title = "{The Energy Dependence of the Centroid Frequency and Phase Lag of the Quasi-periodic Oscillations in GRS 1915+105}",
      journal = {\apj},
     keywords = {accretion, accretion disks, black hole physics, stars: individual: GRS 1915+105, stars: oscillations, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = 2010,
        month = feb,
       volume = {710},
       number = {1},
        pages = {836-842},
          doi = {10.1088/0004-637X/710/1/836},
archivePrefix = {arXiv},
       eprint = {0912.4769},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...710..836Q},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{uttley_causal_2011,
       author = {{Uttley}, P. and {Wilkinson}, T. and {Cassatella}, P. and {Wilms}, J. and {Pottschmidt}, K. and {Hanke}, M. and {B{\"o}ck}, M.},
        title = "{The causal connection between disc and power-law variability in hard state black hole X-ray binaries}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, X-rays: binaries, X-rays: individual: GX 339-4, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2011,
        month = jun,
       volume = {414},
       number = {1},
        pages = {L60-L64},
          doi = {10.1111/j.1745-3933.2011.01056.x},
archivePrefix = {arXiv},
       eprint = {1104.0634},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011MNRAS.414L..60U},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{uttley_causal_2011-1,
	title = {The causal connection between disc and power-law variability in hard state black hole {X}-ray binaries},
	volume = {414},
	doi = {10.1111/j.1745-3933.2011.01056.x},
	number = {1},
	journal = {{\mnras},
	author = {Uttley, P. and Wilkinson, T. and Cassatella, P. and Wilms, J. and Pottschmidt, K. and Hanke, M. and Böck, M.},
	month = jun,
	year = {2011},
	note = {\_eprint: 1104.0634},
	keywords = {X-rays: binaries, Astrophysics - High Energy Astrophysical Phenomena, accretion, accretion discs, Astrophysics - Instrumentation and Methods for Astrophysics, X-rays: individual: GX 339-4},
	pages = {L60--L64},
}
}

@ARTICLE{yuan_hot_2014,
       author = {{Yuan}, Feng and {Narayan}, Ramesh},
        title = "{Hot Accretion Flows Around Black Holes}",
      journal = {\araa},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena},
         year = 2014,
        month = aug,
       volume = {52},
        pages = {529-588},
          doi = {10.1146/annurev-astro-082812-141003},
archivePrefix = {arXiv},
       eprint = {1401.0586},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ARA&A..52..529Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2013MNRAS.433..412L,
       author = {{Li}, Z.~B. and {Zhang}, S. and {Qu}, J.~L. and {Gao}, H.~Q. and {Zhao}, H.~H. and {Huang}, C.~P. and {Song}, L.~M.},
        title = "{The energy dependence of the three types of low-frequency quasi-periodic oscillations in the black hole candidate H1743-322}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, black hole physics, stars: individual: H1743-322, stars: low-mass, stars: oscillations, X-rays: binaries},
         year = 2013,
        month = jul,
       volume = {433},
       number = {1},
        pages = {412-420},
          doi = {10.1093/mnras/stt737},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.433..412L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2013MNRAS.428.1704L,
       author = {{Li}, Z.~B. and {Qu}, J.~L. and {Song}, L.~M. and {Ding}, G.~Q. and {Zhang}, C.~M.},
        title = "{The energy dependence of the centroid frequency of the low-frequency quasi-periodic oscillations in XTE J1550-564}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, black hole physics, stars: individual: XTE J1550-564, stars: low-mass, stars: oscillations, X-rays: binaries},
         year = 2013,
        month = jan,
       volume = {428},
       number = {2},
        pages = {1704-1714},
          doi = {10.1093/mnras/sts149},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.428.1704L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2018ApJ...866..122H,
       author = {{Huang}, Y. and {Qu}, J.~L. and {Zhang}, S.~N. and {Bu}, Q.~C. and {Chen}, Y.~P. and {Tao}, L. and {Zhang}, S. and {Lu}, F.~J. and {Li}, T.~P. and {Song}, L.~M. and {Xu}, Y.~P. and {Cao}, X.~L. and {Chen}, Y. and {Liu}, C.~Z. and {Chang}, H. -K. and {Yu}, W.~F. and {Weng}, S.~S. and {Hou}, X. and {Kong}, A.~K.~H. and {Xie}, F.~G. and {Zhang}, G.~B. and {ZHOU}, J.~F. and {Chang}, Z. and {Chen}, G. and {Chen}, L. and {Chen}, T.~X. and {Chen}, Y.~B. and {Cui}, W. and {Cui}, W.~W. and {Deng}, J.~K. and {Dong}, Y.~W. and {Du}, Y.~Y. and {Fu}, M.~X. and {Gao}, G.~H. and {Gao}, H. and {Gao}, M. and {Ge}, M.~Y. and {Gu}, Y.~D. and {Guan}, J. and {Gungor}, C. and {Guo}, C.~C. and {Han}, D.~W. and {Hu}, W. and {Huo}, J. and {Ji}, J.~F. and {Jia}, S.~M. and {Jiang}, L.~H. and {Jiang}, W.~C. and {Jin}, J. and {Jin}, Y.~J. and {Li}, B. and {Li}, C.~K. and {Li}, G. and {Li}, M.~S. and {Li}, W. and {Li}, X. and {Li}, X.~B. and {Li}, X.~F. and {Li}, Y.~G. and {Li}, Z.~J. and {Li}, Z.~W. and {Liang}, X.~H. and {Liao}, J.~Y. and {Liu}, G.~Q. and {Liu}, H.~W. and {Liu}, S.~Z. and {Liu}, X.~J. and {Liu}, Y. and {Liu}, Y.~N. and {Lu}, B. and {Lu}, X.~F. and {Luo}, T. and {Ma}, X. and {Meng}, B. and {Nang}, Y. and {Nie}, J.~Y. and {Ou}, G. and {Sai}, N. and {Shang}, R.~C. and {Sun}, L. and {Tan}, Y. and {Tao}, W. and {Tuo}, Y.~L. and {Wang}, G.~F. and {Wang}, H.~Y. and {Wang}, J. and {Wang}, W.~S. and {Wang}, Y.~S. and {Wen}, X.~Y. and {Wu}, B.~B. and {Wu}, M. and {Xiao}, G.~C. and {Xiong}, S.~L. and {Xu}, H. and {Yan}, L.~L. and {Yang}, J.~W. and {Yang}, S. and {Yang}, Y.~J. and {Zhang}, A.~M. and {Zhang}, C.~L. and {Zhang}, C.~M. and {Zhang}, F. and {Zhang}, H.~M. and {Zhang}, J. and {Zhang}, Q. and {Zhang}, T. and {Zhang}, W. and {Zhang}, W.~C. and {Zhang}, W.~Z. and {Zhang}, Y. and {Zhang}, Y. and {Zhang}, Y.~F. and {Zhang}, Y.~J. and {Zhang}, Z. and {Zhang}, Z. and {Zhang}, Z.~L. and {Zhao}, H.~S. and {Zhao}, J.~L. and {Zhao}, X.~F. and {Zheng}, S.~J. and {Zhu}, Y. and {Zhu}, Y.~X. and {Zou}, C.~L. and {Insight-HXMT Collaboration}},
        title = "{INSIGHT-HXMT Observations of the New Black Hole Candidate MAXI J1535-571: Timing Analysis}",
      journal = {\apj},
     keywords = {black hole physics, stars: individual: MAXI J1535‑571, X-rays: binaries, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2018,
        month = oct,
       volume = {866},
       number = {2},
          eid = {122},
        pages = {122},
          doi = {10.3847/1538-4357/aade4c},
archivePrefix = {arXiv},
       eprint = {1808.05318},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...866..122H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
} 


@article{yadav_astrosatlaxpc_2016,
	title = {Astrosat/{LAXPC} {Reveals} the {High}-energy {Variability} of {GRS} 1915+105 in the {X} {Class}},
	volume = {833},
	doi = {10.3847/0004-637X/833/1/27},
	number = {1},
	journal = {{\textbackslash}apj},
	author = {Yadav, J. S. and Misra, Ranjeev and Verdhan Chauhan, Jai and Agrawal, P. C. and Antia, H. M. and Pahari, Mayukh and Dedhia, Dhiraj and Katoch, Tilak and Madhwani, P. and Manchanda, R. K. and Paul, B. and Shah, Parag and Ishwara-Chandra, C. H.},
	month = dec,
	year = {2016},
	note = {\_eprint: 1608.07023},
	keywords = {X-rays: binaries, Astrophysics - High Energy Astrophysical Phenomena, black hole physics, accretion, accretion disks},
	pages = {27},
}

@ARTICLE{shakura_black_1973,
       author = {{Shakura}, N.~I. and {Sunyaev}, R.~A.},
        title = "{Black holes in binary systems. Observational appearance.}",
      journal = {\aap},
         year = 1973,
        month = jan,
       volume = {24},
        pages = {337-355},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1973A&A....24..337S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1975ApJ...195L..65B,
       author = {{Bardeen}, James M. and {Petterson}, Jacobus A.},
        title = "{The Lense-Thirring Effect and Accretion Disks around Kerr Black Holes}",
      journal = {\apjl},
         year = 1975,
        month = jan,
       volume = {195},
        pages = {L65},
          doi = {10.1086/181711},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1975ApJ...195L..65B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{lense_uber_1918,
	title = {Über den {Einfluß} der {Eigenrotation} der {Zentralkörper} auf die {Bewegung} der {Planeten} und {Monde} nach der {Einsteinschen} {Gravitationstheorie}},
	volume = {19},
	journal = {Physikalische Zeitschrift},
	author = {Lense, Josef and Thirring, Hans},
	month = jan,
	year = {1918},
	pages = {156},
}

@article{nixon_broken_2012,
	title = {Broken discs: warp propagation in accretion discs},
	volume = {421},
	doi = {10.1111/j.1365-2966.2011.20377.x},
	number = {2},
	journal = {{\textbackslash}mnras},
	author = {Nixon, Christopher J. and King, Andrew R.},
	month = apr,
	year = {2012},
	note = {\_eprint: 1201.1297},
	keywords = {Astrophysics - High Energy Astrophysical Phenomena, black hole physics, accretion, accretion discs, galaxies: active, galaxies: evolution, galaxies: jets},
	pages = {1201--1208},
}
@ARTICLE{2021MNRAS.507..983L,
       author = {{Liska}, M. and {Hesp}, C. and {Tchekhovskoy}, A. and {Ingram}, A. and {van der Klis}, M. and {Markoff}, S.~B. and {Van Moer}, M.},
        title = "{Disc tearing and Bardeen-Petterson alignment in GRMHD simulations of highly tilted thin accretion discs}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, black hole physics, MHD, methods: numerical, galaxies: jets, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = oct,
       volume = {507},
       number = {1},
        pages = {983-990},
          doi = {10.1093/mnras/staa099},
archivePrefix = {arXiv},
       eprint = {1904.08428},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.507..983L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{van_den_eijnden_probing_2016,
	title = {Probing the origin of quasi-periodic oscillations: the short-time-scale evolution of phase lags in {GRS} 1915+105},
	volume = {458},
	doi = {10.1093/mnras/stw610},
	number = {4},
	journal = {{\textbackslash}mnras},
	author = {van den Eijnden, Jakob and Ingram, Adam and Uttley, Phil},
	month = jun,
	year = {2016},
	note = {\_eprint: 1603.03392},
	keywords = {Astrophysics - High Energy Astrophysical Phenomena, black hole physics, accretion, accretion discs, X-rays: individual: GRS 1915+105},
	pages = {3655--3666},
}


@article{2017ApJ...834...90H,
       author = {{Huppenkothen}, D. and {Younes}, G. and {Ingram}, A. and {Kouveliotou}, C. and {G{\"o}{\u{g}}{\"u}{\c{s}}}, E. and {Bachetti}, M. and {S{\'a}nchez-Fern{\'a}ndez}, C. and {Chenevez}, J. and {Motta}, S. and {van der Klis}, M. and {Granot}, J. and {Gehrels}, N. and {Kuulkers}, E. and {Tomsick}, J.~A. and {Walton}, D.~J.},
        title = "{Detection of Very Low-frequency, Quasi-periodic Oscillations in the 2015 Outburst of V404 Cygni}",
      journal = {\apj},
     keywords = {methods: statistical, relativistic processes, stars: black holes, X-rays: binaries, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2017,
        month = jan,
       volume = {834},
       number = {1},
          eid = {90},
        pages = {90},
          doi = {10.3847/1538-4357/834/1/90},
archivePrefix = {arXiv},
       eprint = {1610.08653},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...834...90H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{janiuk_time-delays_2005,
	title = {Time-delays between the soft and hard {X}-ray bands in {GRS} 1915+105},
	volume = {356},
	doi = {10.1111/j.1365-2966.2004.08435.x},
	number = {1},
	journal = {{\textbackslash}mnras},
	author = {Janiuk, A. and Czerny, B.},
	month = jan,
	year = {2005},
	note = {\_eprint: astro-ph/0409671},
	keywords = {Astrophysics, black hole physics, accretion, accretion discs, binaries: close, instabilities, stars: individual: GRS 1915+105, X-rays: stars},
	pages = {205--216},
}

@article{uttley_causal_2011-2,
	title = {The causal connection between disc and power-law variability in hard state black hole {X}-ray binaries},
	volume = {414},
	doi = {10.1111/j.1745-3933.2011.01056.x},
	number = {1},
	journal = {{\textbackslash}mnras},
	author = {Uttley, P. and Wilkinson, T. and Cassatella, P. and Wilms, J. and Pottschmidt, K. and Hanke, M. and Böck, M.},
	month = jun,
	year = {2011},
	note = {\_eprint: 1104.0634},
	keywords = {X-rays: binaries, Astrophysics - High Energy Astrophysical Phenomena, accretion, accretion discs, Astrophysics - Instrumentation and Methods for Astrophysics, X-rays: individual: GX 339-4},
	pages = {L60--L64},
}

@ARTICLE{1997MNRAS.292..679L,
       author = {{Lyubarskii}, Yu. E.},
        title = "{Flicker noise in accretion discs}",
      journal = {\mnras},
     keywords = {Accretion Disks, Noise Measurement, Mass Transfer, Luminosity, X Ray Sources, Computational Astrophysics, Radial Distribution, Astrophysics, ACCRETION, ACCRETION DISCS, X-RAYS: GENERAL},
         year = 1997,
        month = dec,
       volume = {292},
       number = {3},
        pages = {679-685},
          doi = {10.1093/mnras/292.3.679},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997MNRAS.292..679L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{yang_insight-hxmt_2022,
	title = {An {Insight}-{HXMT} view of the {mHz} quasi-regular modulation phenomenon in the black hole {X}-ray binary {4U} 1630-47},
	journal = {arXiv e-prints},
	author = {Yang, Zi-Xu and Zhang, Liang and Huang, Yue and Bu, Qingcui and Zhang, Zhen and Liu, He-Xin and Yu, Wei and Wang, Peng-Ju and Zhao, Q. C. and Tao, L. and Qu, Jin-Lu and Zhang, Shu and Zhang, Shuang-Nan and Song, Liming and Lu, Fangjun and Cao, Xuelei and Chen, Li and Cai, Ce and Chang, Zhi and Chen, Tianxian and Chen, Yong and Chen, Yupeng and Chen, Yibao and Cui, Weiwei and Ding, Guoqiang and Du, Yuanyuan and Gao, GuanHua and Gao, He and Ge, Mingyu and Gu, Yudong and Guan, Ju and Guo, Chengcheng and Han, Dawei and Huo, Jia and Jia, Shumei and Jiang, Weichun and Jin, Jing and Kong, Lingda and Li, Bing and Li, Gang and Li, Wei and Li, Xian and Li, Xufang and Li, Zhengwei and Li, Chengkui and Lin, Lin and Liu, Congzhan and Li, Tipei and Li, Xiaobo and Liang, Xiaohua and Liao, Jinyuan and Liu, Hongwei and Liu, Xiaojing and Lu, Xuefeng and Luo, Qi and Luo, Tao and Ma, Binyuan and Ma, Ruican and Ma, Xiang and Meng, Bin and Nang, Yi and Nie, Jianyin and Ou, Ge and Ren, Xiaoqin and Sai, Na and Song, Xinying and Sun, Liang and Tan, Ying and Tuo, Youli and Wang, Chen and Wang, Wenshuai and Wang, Lingjun and Wang, Yusa and Wang, Jieshuang and Wen, Xiangyang and Wu, Bobing and Wu, Baiyang and Wu, Mei and Xiao, Shuo and Xu, Yupeng and Xiong, Shaolin and Yang, Sheng and Yang, Yanji and Yi, Qibin and Yin, Qianqing and You, Yuan and Zhang, Bing and Zhang, Fan and Zhang, Hongmei and Zhang, Juan and Zhang, Wanchang and Zhang, Wei and Zhang, Binbin and Zhang, Peng and Zhang, Yifei and Zhang, Yuanhang and Zhao, Haisheng and Zhao, Xiaofan and Zheng, Shijie and Zhou, Dengke},
	month = jul,
	year = {2022},
	note = {\_eprint: 2207.14048},
	keywords = {Astrophysics - High Energy Astrophysical Phenomena},
	pages = {arXiv:2207.14048},
}



@ARTICLE{2021ApJ...919...92B,
       author = {{Bu}, Q.~C. and {Zhang}, S.~N. and {Santangelo}, A. and {Belloni}, T.~M. and {Zhang}, L. and {Qu}, J.~L. and {Tao}, L. and {Huang}, Y. and {Ma}, X. and {Li}, Z.~S. and {Zhang}, S. and {Chen}, L. and {Cai}, C. and {Cao}, X.~L. and {Chang}, Z. and {Chen}, T.~X. and {Chen}, Y. and {Chen}, Y.~P. and {Cui}, W.~W. and {Du}, Y.~Y. and {Gao}, G.~H. and {Gao}, H. and {Ge}, M.~Y. and {Gu}, Y.~D. and {Guan}, J. and {Guo}, C.~C. and {Han}, D.~W. and {Huo}, J. and {Jia}, S.~M. and {Jiang}, W.~C. and {Jin}, J. and {Kong}, L.~D. and {Li}, B. and {Li}, C.~K. and {Li}, G. and {Li}, T.~P. and {Li}, W. and {Li}, X. and {Li}, X.~B. and {Li}, X.~F. and {Li}, Z.~W. and {Liang}, X.~H. and {Liao}, J.~Y. and {Liu}, C.~Z. and {Liu}, H.~X. and {Liu}, H.~W. and {Liu}, X.~J. and {Lu}, F.~J. and {Lu}, X.~F. and {Luo}, Q. and {Luo}, T. and {Ma}, R.~C. and {Meng}, B. and {Nang}, Y. and {Nie}, J.~Y. and {Ou}, G. and {Sai}, N. and {Song}, L.~M. and {Song}, X.~Y. and {Sun}, L. and {Tan}, Y. and {Tuo}, Y.~L. and {Wang}, C. and {Wang}, L.~J. and {Wang}, P.~J. and {Wang}, W.~S. and {Wang}, Y.~S. and {Wen}, X.~Y. and {Wu}, B.~Y. and {Wu}, B.~B. and {Wu}, M. and {Xiao}, G.~C. and {Xiao}, S. and {Xiong}, S.~L. and {Xu}, Y.~P. and {Yang}, S. and {Yang}, Y.~J. and {Yi}, Q.~B. and {Yin}, Q.~Q. and {You}, Y. and {Zhang}, F. and {Zhang}, H.~M. and {Zhang}, J. and {Zhang}, P. and {Zhang}, W.~C. and {Zhang}, W. and {Zhang}, Y.~F. and {Zhang}, Y.~H. and {Zhao}, H.~S. and {Zhao}, X.~F. and {Zheng}, S.~J. and {Zhou}, D.~K. and {Insight-HMXT Collaboration}},
        title = "{Broadband Variability Study of Maxi J1631-479 in Its Hard-intermediate State Observed with Insight-HXMT}",
      journal = {\apj},
     keywords = {Stellar accretion disks, Low-mass x-ray binary stars, Black hole physics, 1579, 939, 159, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2021,
        month = oct,
       volume = {919},
       number = {2},
          eid = {92},
        pages = {92},
          doi = {10.3847/1538-4357/ac11f5},
archivePrefix = {arXiv},
       eprint = {2107.06333},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...919...92B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2012MNRAS.421.1201N,
       author = {{Nixon}, Christopher J. and {King}, Andrew R.},
        title = "{Broken discs: warp propagation in accretion discs}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, black hole physics, galaxies: active, galaxies: evolution, galaxies: jets, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2012,
        month = apr,
       volume = {421},
       number = {2},
        pages = {1201-1208},
          doi = {10.1111/j.1365-2966.2011.20377.x},
archivePrefix = {arXiv},
       eprint = {1201.1297},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012MNRAS.421.1201N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2013ApJ...771..101P,
       author = {{Pasham}, Dheeraj R. and {Strohmayer}, Tod E.},
        title = "{On the Nature of the mHz X-Ray Quasi-periodic Oscillations from Ultraluminous X-Ray Source M82 X-1: Search for Timing-Spectral Correlations}",
      journal = {\apj},
     keywords = {accretion, accretion disks, methods: data analysis, X-rays: binaries, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2013,
        month = jul,
       volume = {771},
       number = {2},
          eid = {101},
        pages = {101},
          doi = {10.1088/0004-637X/771/2/101},
archivePrefix = {arXiv},
       eprint = {1308.1677},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...771..101P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2016ApJ...833...27Y,
       author = {{Yadav}, J.~S. and {Misra}, Ranjeev and {Verdhan Chauhan}, Jai and {Agrawal}, P.~C. and {Antia}, H.~M. and {Pahari}, Mayukh and {Dedhia}, Dhiraj and {Katoch}, Tilak and {Madhwani}, P. and {Manchanda}, R.~K. and {Paul}, B. and {Shah}, Parag and {Ishwara-Chandra}, C.~H.},
        title = "{Astrosat/LAXPC Reveals the High-energy Variability of GRS 1915+105 in the X Class}",
      journal = {\apj},
     keywords = {accretion, accretion disks, black hole physics, X-rays: binaries, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2016,
        month = dec,
       volume = {833},
       number = {1},
          eid = {27},
        pages = {27},
          doi = {10.3847/0004-637X/833/1/27},
archivePrefix = {arXiv},
       eprint = {1608.07023},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...833...27Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016MNRAS.458.3655V,
       author = {{van den Eijnden}, Jakob and {Ingram}, Adam and {Uttley}, Phil},
        title = "{Probing the origin of quasi-periodic oscillations: the short-time-scale evolution of phase lags in GRS 1915+105}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, black hole physics, X-rays: individual: GRS 1915+105, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2016,
        month = jun,
       volume = {458},
       number = {4},
        pages = {3655-3666},
          doi = {10.1093/mnras/stw610},
archivePrefix = {arXiv},
       eprint = {1603.03392},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.458.3655V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1994ApJS...92..511V,
       author = {{van der Klis}, M.},
        title = "{Similarities in Neutron Star and Black Hole Accretion}",
      journal = {\apjs},
     keywords = {Black Holes (Astronomy), Neutron Stars, Stellar Mass Accretion, X Ray Astronomy, X Ray Binaries, X Ray Spectra, Color-Color Diagram, Light Curve, Power Spectra, Stellar Oscillations, Astronomy, ACCRETION, ACCRETION DISKS, BLACK HOLE PHYSICS, STARS: NEUTRON},
         year = 1994,
        month = jun,
       volume = {92},
        pages = {511},
          doi = {10.1086/192006},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1994ApJS...92..511V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016MNRAS.457.2999M,
       author = {{Mir}, Mubashir Hamid and {Misra}, Ranjeev and {Pahari}, Mayukh and {Iqbal}, Naseer and {Ahmad}, Naveel},
        title = "{A model for the energy-dependent time-lag and rms of the heartbeat oscillations in GRS 1915+105}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, black hole physics, X-rays: binaries, X-rays: individual: GRS 1915+105, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2016,
        month = apr,
       volume = {457},
       number = {3},
        pages = {2999-3005},
          doi = {10.1093/mnras/stw156},
archivePrefix = {arXiv},
       eprint = {1601.04870},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.457.2999M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2020MNRAS.498.2757G,
       author = {{Garg}, Akash and {Misra}, Ranjeev and {Sen}, Somasri},
        title = "{Identifying the radiative components responsible for quasi-periodic oscillations of black hole systems}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, black hole physics, X-rays: binaries, X-rays: individual: GRS 1915+105, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = oct,
       volume = {498},
       number = {2},
        pages = {2757-2765},
          doi = {10.1093/mnras/staa2506},
archivePrefix = {arXiv},
       eprint = {2008.06468},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.498.2757G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2014ApJ...782...76G,
       author = {{Garc{\'\i}a}, J. and {Dauser}, T. and {Lohfink}, A. and {Kallman}, T.~R. and {Steiner}, J.~F. and {McClintock}, J.~E. and {Brenneman}, L. and {Wilms}, J. and {Eikmann}, W. and {Reynolds}, C.~S. and {Tombesi}, F.},
        title = "{Improved Reflection Models of Black Hole Accretion Disks: Treating the Angular Distribution of X-Rays}",
      journal = {\apj},
     keywords = {accretion, accretion disks, black hole physics, galaxies: individual: Ark 120, line: formation, radiative transfer, X-rays: general, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2014,
        month = feb,
       volume = {782},
       number = {2},
          eid = {76},
        pages = {76},
          doi = {10.1088/0004-637X/782/2/76},
archivePrefix = {arXiv},
       eprint = {1312.3231},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...782...76G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2015ApJ...808L..37G,
       author = {{Garc{\'\i}a}, Javier A. and {Dauser}, Thomas and {Steiner}, James F. and {McClintock}, Jeffrey E. and {Keck}, Mason L. and {Wilms}, J{\"o}rn},
        title = "{On Estimating the High-energy Cutoff in the X-Ray Spectra of Black Holes via Reflection Spectroscopy}",
      journal = {\apjl},
     keywords = {accretion, accretion disks, atomic processes, black hole physics, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = aug,
       volume = {808},
       number = {2},
          eid = {L37},
        pages = {L37},
          doi = {10.1088/2041-8205/808/2/L37},
archivePrefix = {arXiv},
       eprint = {1505.03616},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...808L..37G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2021ApJ...909..146C,
       author = {{Connors}, Riley M.~T. and {Garc{\'\i}a}, Javier A. and {Tomsick}, John and {Hare}, Jeremy and {Dauser}, Thomas and {Grinberg}, Victoria and {Steiner}, James F. and {Mastroserio}, Guglielmo and {Sridhar}, Navin and {Fabian}, Andrew C. and {Jiang}, Jiachen and {Parker}, Michael L. and {Harrison}, Fiona and {Kallman}, Timothy R.},
        title = "{Reflection Modeling of the Black Hole Binary 4U 1630-47: The Disk Density and Returning Radiation}",
      journal = {\apj},
     keywords = {Accretion, Stellar accretion disks, black hole physics, Atomic physics, Low-mass x-ray binary stars, 14, 1579, 159, 2063, 939, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2021,
        month = mar,
       volume = {909},
       number = {2},
          eid = {146},
        pages = {146},
          doi = {10.3847/1538-4357/abdd2c},
archivePrefix = {arXiv},
       eprint = {2101.06343},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...909..146C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010ApJ...718..695G,
       author = {{Garc{\'\i}a}, J. and {Kallman}, T.~R.},
        title = "{X-ray Reflected Spectra from Accretion Disk Models. I. Constant Density Atmospheres}",
      journal = {\apj},
     keywords = {accretion, accretion disks, atomic processes, black hole physics, line: formation, radiative transfer, X-rays: general, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2010,
        month = aug,
       volume = {718},
       number = {2},
        pages = {695-706},
          doi = {10.1088/0004-637X/718/2/695},
archivePrefix = {arXiv},
       eprint = {1006.0485},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...718..695G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2020ApJ...890...53S,
       author = {{Sridhar}, Navin and {Garc{\'\i}a}, Javier A. and {Steiner}, James F. and {Connors}, Riley M.~T. and {Grinberg}, Victoria and {Harrison}, Fiona A.},
        title = "{Evolution of the Accretion Disk-Corona during the Bright Hard-to-soft State Transition: A Reflection Spectroscopic Study with GX 339-4}",
      journal = {\apj},
     keywords = {High energy astrophysics, Compact objects, Black hole physics, Low-mass x-ray binary stars, Accretion, X-ray astronomy, Spectroscopy, Astronomy data modeling, X-ray sources, General relativity, Gravitation, Astrophysical black holes, 739, 288, 159, 939, 14, 1810, 1558, 1859, 1822, 641, 661, 98, Astrophysics - High Energy Astrophysical Phenomena, General Relativity and Quantum Cosmology, High Energy Physics - Experiment, Physics - Data Analysis, Statistics and Probability, Physics - Plasma Physics},
         year = 2020,
        month = feb,
       volume = {890},
       number = {1},
          eid = {53},
        pages = {53},
          doi = {10.3847/1538-4357/ab64f5},
archivePrefix = {arXiv},
       eprint = {1912.11447},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...890...53S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{1989MNRAS.238..729F,
       author = {{Fabian}, A.~C. and {Rees}, M.~J. and {Stella}, L. and {White}, N.~E.},
        title = "{X-ray fluorescence from the inner disc in Cygnus X-1.}",
      journal = {\mnras},
     keywords = {Accretion Disks, Black Holes (Astronomy), Cygnus Constellation, X Ray Fluorescence, X Ray Spectra, Black Body Radiation, Emission Spectra, Line Spectra, Red Shift, Astrophysics},
         year = 1989,
        month = may,
       volume = {238},
        pages = {729-736},
          doi = {10.1093/mnras/238.3.729},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1989MNRAS.238..729F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2021MNRAS.508..287S,
       author = {{Shui}, Q.~C. and {Yin}, H.~X. and {Zhang}, S. and {Qu}, J.~L. and {Chen}, Y.~P. and {Kong}, L.~D. and {Wang}, P.~J. and {Zhang}, H.~F. and {Song}, J.~X. and {Ning}, B. and {Wang}, Y.~F. and {Chang}, Z. and {Zhang}, P.},
        title = "{State transitions of GX 339-4 during its outburst rising phase}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, black hole physics, binaries: close, X-rays: binaries, X-rays: individual: GX 339-4, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2021,
        month = nov,
       volume = {508},
       number = {1},
        pages = {287-299},
          doi = {10.1093/mnras/stab2521},
archivePrefix = {arXiv},
       eprint = {2109.02088},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.508..287S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{Yang_2022,
	doi = {10.3847/1538-4357/ac84d6},
	url = {https://doi.org/10.3847/1538-4357/ac84d6},
	year = 2022,
	month = {sep},
	publisher = {American Astronomical Society},
	volume = {937},
	number = {1},
	pages = {33},
	author = {Zi-xu Yang and Liang Zhang and Yue Huang and Qingcui Bu and Zhen Zhang and He-Xin Liu and Wei Yu and Peng-Ju Wang and Q. C. Zhao and L. Tao and Jin-Lu Qu and Shu Zhang and Shuang-Nan Zhang and Liming Song and Fangjun Lu and Xuelei Cao and Li Chen and Ce Cai and Zhi Chang and Tianxiang Chen and Yong Chen and Yupeng Chen and Yibao Chen and Weiwei Cui and Guoqiang Ding and Yuanyuan Du and Guanhua Gao and He Gao and Mingyu Ge and Yudong Gu and Ju Guan and Chengcheng Guo and Dawei Han and Jia Huo and Shumei Jia and Weichun Jiang and Jing Jin and Lingda Kong and Bing Li and Gang Li and Wei Li and Xian Li and Xufang Li and Zhengwei Li and Chengkui Li and Lin Lin and Congzhan Liu and Tipei Li and Xiaobo Li and Xiaohua Liang and Jinyuan Liao and Hongwei Liu and Xiaojing Liu and Xuefeng Lu and Qi Luo and Tao Luo and Binyuan Ma and RuiCan Ma and Xiang Ma and Bin Meng and Yi Nang and Jianyin Nie and Ge Ou and Xiaoqin Ren and Na Sai and Xinying Song and Liang Sun and Ying Tan and Youli Tuo and Chen Wang and Wenshuai Wang and Lingjun Wang and Yusa Wang and Jieshuang Wang and Xiangyang Wen and Bobing Wu and Baiyang Wu and Mei Wu and Shuo Xiao and Yupeng Xu and Shaolin Xiong and Sheng Yang and Yanji Yang and Qibin Yi and Qianqing Yin and Yuan You and Bing Zhang and Fan Zhang and Hongmei Zhang and Juan Zhang and Wanchang Zhang and Wei Zhang and Binbin Zhang and Peng Zhang and Yifei Zhang and Yuanhang Zhang and Haisheng Zhao and Xiaofan Zhao and Shijie Zheng and Dengke Zhou},
	title = {An Insight-{HXMT} View of the {mHz} Quasi-regular Modulation Phenomenon in the Black Hole X-Ray Binary 4U 1630{\textendash}47},
	journal = {The Astrophysical Journal},
}
@ARTICLE{2022ApJ...937...33Y,
       author = {{Yang}, Zi-xu and {Zhang}, Liang and {Huang}, Yue and {Bu}, Qingcui and {Zhang}, Zhen and {Liu}, He-Xin and {Yu}, Wei and {Wang}, Peng-Ju and {Zhao}, Q.~C. and {Tao}, L. and {Qu}, Jin-Lu and {Zhang}, Shu and {Zhang}, Shuang-Nan and {Song}, Liming and {Lu}, Fangjun and {Cao}, Xuelei and {Chen}, Li and {Cai}, Ce and {Chang}, Zhi and {Chen}, Tianxiang and {Chen}, Yong and {Chen}, Yupeng and {Chen}, Yibao and {Cui}, Weiwei and {Ding}, Guoqiang and {Du}, Yuanyuan and {Gao}, Guanhua and {Gao}, He and {Ge}, Mingyu and {Gu}, Yudong and {Guan}, Ju and {Guo}, Chengcheng and {Han}, Dawei and {Huo}, Jia and {Jia}, Shumei and {Jiang}, Weichun and {Jin}, Jing and {Kong}, Lingda and {Li}, Bing and {Li}, Gang and {Li}, Wei and {Li}, Xian and {Li}, Xufang and {Li}, Zhengwei and {Li}, Chengkui and {Lin}, Lin and {Liu}, Congzhan and {Li}, Tipei and {Li}, Xiaobo and {Liang}, Xiaohua and {Liao}, Jinyuan and {Liu}, Hongwei and {Liu}, Xiaojing and {Lu}, Xuefeng and {Luo}, Qi and {Luo}, Tao and {Ma}, Binyuan and {Ma}, RuiCan and {Ma}, Xiang and {Meng}, Bin and {Nang}, Yi and {Nie}, Jianyin and {Ou}, Ge and {Ren}, Xiaoqin and {Sai}, Na and {Song}, Xinying and {Sun}, Liang and {Tan}, Ying and {Tuo}, Youli and {Wang}, Chen and {Wang}, Wenshuai and {Wang}, Lingjun and {Wang}, Yusa and {Wang}, Jieshuang and {Wen}, Xiangyang and {Wu}, Bobing and {Wu}, Baiyang and {Wu}, Mei and {Xiao}, Shuo and {Xu}, Yupeng and {Xiong}, Shaolin and {Yang}, Sheng and {Yang}, Yanji and {Yi}, Qibin and {Yin}, Qianqing and {You}, Yuan and {Zhang}, Bing and {Zhang}, Fan and {Zhang}, Hongmei and {Zhang}, Juan and {Zhang}, Wanchang and {Zhang}, Wei and {Zhang}, Binbin and {Zhang}, Peng and {Zhang}, Yifei and {Zhang}, Yuanhang and {Zhao}, Haisheng and {Zhao}, Xiaofan and {Zheng}, Shijie and {Zhou}, Dengke},
        title = "{An Insight-HXMT View of the mHz Quasi-regular Modulation Phenomenon in the Black Hole X-Ray Binary 4U 1630-47}",
      journal = {\apj},
     keywords = {Accretion, Astrophysical black holes, Low-mass x-ray binary stars, Stellar mass black holes, 14, 98, 939, 1611, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2022,
        month = sep,
       volume = {937},
       number = {1},
          eid = {33},
        pages = {33},
          doi = {10.3847/1538-4357/ac84d6},
archivePrefix = {arXiv},
       eprint = {2207.14048},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022ApJ...937...33Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2000A&A...355..271B,
       author = {{Belloni}, T. and {Klein-Wolt}, M. and {M{\'e}ndez}, M. and {van der Klis}, M. and {van Paradijs}, J.},
        title = "{A model-independent analysis of the variability of GRS 1915+105}",
      journal = {\aap},
     keywords = {BLACK HOLE PHYSICS, STARS: BINARIES: CLOSE, STARS: INDIVIDUAL: GRS 1915+105, X-RAYS: STARS, Astrophysics},
         year = 2000,
        month = mar,
       volume = {355},
        pages = {271-290},
archivePrefix = {arXiv},
       eprint = {astro-ph/0001103},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000A&A...355..271B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2002MNRAS.331..745K,
       author = {{Klein-Wolt}, M. and {Fender}, R.~P. and {Pooley}, G.~G. and {Belloni}, T. and {Migliari}, S. and {Morgan}, E.~H. and {van der Klis}, M.},
        title = "{Hard X-ray states and radio emission in GRS 1915+105}",
      journal = {\mnras},
     keywords = {binaries: close, stars: individual: GRS 1915+105, radio continuum: stars, X-rays: individual: GRS 1915+105, Astrophysics},
         year = 2002,
        month = apr,
       volume = {331},
       number = {3},
        pages = {745-764},
          doi = {10.1046/j.1365-8711.2002.05223.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0112044},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002MNRAS.331..745K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2011ApJ...737...69N,
       author = {{Neilsen}, Joseph and {Remillard}, Ronald A. and {Lee}, Julia C.},
        title = "{The Physics of the ``Heartbeat'' State of GRS 1915+105}",
      journal = {\apj},
     keywords = {accretion, accretion disks, binaries: close, black hole physics, instabilities, stars: winds, outflows, X-rays: individual: GRS 1915+105, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2011,
        month = aug,
       volume = {737},
       number = {2},
          eid = {69},
        pages = {69},
          doi = {10.1088/0004-637X/737/2/69},
archivePrefix = {arXiv},
       eprint = {1106.0298},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...737...69N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1996ASPC..101...17A,
       author = {{Arnaud}, K.~A.},
        title = "{XSPEC: The First Ten Years}",
    booktitle = {Astronomical Data Analysis Software and Systems V},
         year = 1996,
       editor = {{Jacoby}, George H. and {Barnes}, Jeannette},
       series = {Astronomical Society of the Pacific Conference Series},
       volume = {101},
        month = jan,
        pages = {17},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996ASPC..101...17A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2007MNRAS.376.1740K,
       author = {{King}, A.~R. and {Pringle}, J.~E. and {Livio}, M.},
        title = "{Accretion disc viscosity: how big is alpha?}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, Astrophysics},
         year = 2007,
        month = apr,
       volume = {376},
       number = {4},
        pages = {1740-1746},
          doi = {10.1111/j.1365-2966.2007.11556.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0701803},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007MNRAS.376.1740K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014MNRAS.437.3994N,
       author = {{Nixon}, Chris and {Salvesen}, Greg},
        title = "{A physical model for state transitions in black hole X-ray binaries}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, black hole physics, hydrodynamics, X-rays: binaries, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2014,
        month = feb,
       volume = {437},
       number = {4},
        pages = {3994-3999},
          doi = {10.1093/mnras/stt2215},
archivePrefix = {arXiv},
       eprint = {1311.2930},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.437.3994N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2022RAA....22k5002F,
       author = {{Fu}, Yu-Cong and {Song}, L.~M. and {Ding}, G.~Q. and {Zhang}, S.~N. and {Qu}, J.~L. and {Zhang}, S. and {Zhang}, L. and {Bu}, Q.~C. and {Huang}, Y. and {Ma}, X. and {Yang}, Z.~X. and {Tuo}, Y.~L. and {Lu}, X.~F. and {Zhou}, D.~K. and {Wu}, B.~Y. and {Li}, T.~M. and {Xu}, Y.~C.},
        title = "{Spectral and Timing Analysis of the Black Hole Transient MAXI J1631-479 During its 2019 Outburst Observed with Insight-HXMT}",
      journal = {RAA},
     keywords = {accretion, accretion disks, stars: black holes, X-rays: binaries},
         year = 2022,
        month = nov,
       volume = {22},
       number = {11},
          eid = {115002},
        pages = {115002},
          doi = {10.1088/1674-4527/ac8d80},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022RAA....22k5002F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2015MNRAS.449.1251D,
       author = {{Do{\u{g}}an}, Suzan and {Nixon}, Chris and {King}, Andrew and {Price}, Daniel J.},
        title = "{Tearing up a misaligned accretion disc with a binary companion}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, black hole physics, hydrodynamics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2015,
        month = may,
       volume = {449},
       number = {2},
        pages = {1251-1258},
          doi = {10.1093/mnras/stv347},
archivePrefix = {arXiv},
       eprint = {1502.05410},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.449.1251D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2001ApJ...553..955F,
       author = {{Fragile}, P. Chris and {Mathews}, Grant J. and {Wilson}, James R.},
        title = "{Bardeen-Petterson Effect and Quasi-periodic Oscillations in X-Ray Binaries}",
      journal = {\apj},
     keywords = {Accretion, Accretion Disks, Black Hole Physics, stars: individual (GRO J1655-40), Stars: Neutron, X-Rays: Stars, Astrophysics},
         year = 2001,
        month = jun,
       volume = {553},
       number = {2},
        pages = {955-959},
          doi = {10.1086/320990},
archivePrefix = {arXiv},
       eprint = {astro-ph/0007478},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001ApJ...553..955F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013Sci...339...49M,
       author = {{McKinney}, Jonathan C. and {Tchekhovskoy}, Alexander and {Blandford}, Roger D.},
        title = "{Alignment of Magnetized Accretion Disks and Relativistic Jets with Spinning Black Holes}",
      journal = {Science},
     keywords = {ASTRONOMY, Astrophysics - Cosmology and Extragalactic Astrophysics, Astrophysics - High Energy Astrophysical Phenomena, General Relativity and Quantum Cosmology},
         year = 2013,
        month = jan,
       volume = {339},
       number = {6115},
        pages = {49},
          doi = {10.1126/science.1230811},
archivePrefix = {arXiv},
       eprint = {1211.3651},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013Sci...339...49M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@INPROCEEDINGS{2016ASSL..440...61B,
       author = {{Belloni}, Tomaso M. and {Motta}, Sara E.},
        title = "{Transient Black Hole Binaries}",
     keywords = {Physics, Astrophysics - High Energy Astrophysical Phenomena},
    booktitle = {Astrophysics of Black Holes: From Fundamental Aspects to Latest Developments},
         year = 2016,
       editor = {{Bambi}, Cosimo},
       series = {Astrophysics and Space Science Library},
       volume = {440},
        month = jan,
        pages = {61},
          doi = {10.1007/978-3-662-52859-4_2},
archivePrefix = {arXiv},
       eprint = {1603.07872},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ASSL..440...61B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018MNRAS.474L..81L,
       author = {{Liska}, M. and {Hesp}, C. and {Tchekhovskoy}, A. and {Ingram}, A. and {van der Klis}, M. and {Markoff}, S.},
        title = "{Formation of precessing jets by tilted black hole discs in 3D general relativistic MHD simulations}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, black hole physics, MHD, methods: numerical, galaxies: jets, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics, General Relativity and Quantum Cosmology},
         year = 2018,
        month = feb,
       volume = {474},
       number = {1},
        pages = {L81-L85},
          doi = {10.1093/mnrasl/slx174},
archivePrefix = {arXiv},
       eprint = {1707.06619},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.474L..81L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2023arXiv230300481M,
       author = {{Ma}, X. and {Zhang}, L. and {Tao}, L. and {Bu}, Q.~C. and {Qu}, J.~L. and {Zhang}, S.~N. and {Zhou}, D.~K. and {Huang}, Y. and {Jia}, S.~M. and {Song}, L.~M. and {Zhang}, S. and {Ge}, M.~Y. and {Liu}, H.~X. and {Yang}, Z.~X. and {Yu}, W. and {Yorgancioglu}, E.~S.},
        title = "{A detailed view of low-frequency quasi-periodic oscillation in the broadband 0.2-200 keV with Insight-HXMT and NICER}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena},
         year = 2023,
        month = mar,
          eid = {arXiv:2303.00481},
        pages = {arXiv:2303.00481},
          doi = {10.48550/arXiv.2303.00481},
archivePrefix = {arXiv},
       eprint = {2303.00481},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023arXiv230300481M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2022A&A...662A.118M,
       author = {{Mastichiadis}, A. and {Petropoulou}, M. and {Kylafis}, N.~D.},
        title = "{A study of natural frequencies in a dynamic corona - disk system}",
      journal = {\aap},
     keywords = {X-rays: binaries, radiation: dynamics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2022,
        month = jun,
       volume = {662},
          eid = {A118},
        pages = {A118},
          doi = {10.1051/0004-6361/202243397},
archivePrefix = {arXiv},
       eprint = {2204.14139},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022A&A...662A.118M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2022NatAs...6..577M,
       author = {{M{\'e}ndez}, Mariano and {Karpouzas}, Konstantinos and {Garc{\'\i}a}, Federico and {Zhang}, Liang and {Zhang}, Yuexin and {Belloni}, Tomaso M. and {Altamirano}, Diego},
        title = "{Coupling between the accreting corona and the relativistic jet in the microquasar GRS 1915+105}",
      journal = {Nature Astronomy},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena},
         year = 2022,
        month = mar,
       volume = {6},
        pages = {577-583},
          doi = {10.1038/s41550-022-01617-y},
archivePrefix = {arXiv},
       eprint = {2203.02963},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022NatAs...6..577M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2022MNRAS.515.2099B,
       author = {{Bellavita}, Candela and {Garc{\'\i}a}, Federico and {M{\'e}ndez}, Mariano and {Karpouzas}, Konstantinos},
        title = "{vKompth: a variable Comptonization model for low-frequency quasi-periodic oscillations in black hole X-ray binaries}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, black hole physics, X-rays: binaries, X-rays: individual: MAXI J1348-630, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2022,
        month = sep,
       volume = {515},
       number = {2},
        pages = {2099-2109},
          doi = {10.1093/mnras/stac1922},
archivePrefix = {arXiv},
       eprint = {2206.13609},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.515.2099B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2022MNRAS.513.4196G,
       author = {{Garc{\'\i}a}, Federico and {Karpouzas}, Konstantinos and {M{\'e}ndez}, Mariano and {Zhang}, Liang and {Zhang}, Yuexin and {Belloni}, Tomaso and {Altamirano}, Diego},
        title = "{The evolving properties of the corona of GRS 1915+105: a spectral-timing perspective through variable-Comptonization modelling}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, X-ray: binaries, X-ray: individual (GRS 1915+105), Astrophysics - High Energy Astrophysical Phenomena},
         year = 2022,
        month = jul,
       volume = {513},
       number = {3},
        pages = {4196-4207},
          doi = {10.1093/mnras/stac1202},
archivePrefix = {arXiv},
       eprint = {2204.13279},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.513.4196G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






